Requirements Strategy for Managing Human Factors in Automated Vehicle Development

The integration of human factors (HF) knowledge is crucial when developing safety-critical systems, such as automated vehicles (AVs). Ensuring that HF knowledge is considered continuously throughout the AV development process is essential for several reasons, including efficacy, safety, and acceptance of these advanced systems. However, it is challenging to include HF as requirements in agile development. Recently, Requirements Strategies have been suggested to address requirements engineering challenges in agile development. By applying the concept of Requirements Strategies as a lens to the investigation of HF requirements in agile development of AVs, this paper arrives at three areas for investigation: a) ownership and responsibility for HF requirements, b) structure of HF requirements and information models, and c) definition of work and feature flows related to HF requirements. Based on 13 semi-structured interviews with professionals from the global automotive industry, we provide qualitative insights in these three areas. The diverse perspectives and experiences shared by the interviewees provide insightful views and helped to reason about the potential solution spaces in each area for integrating HF within the industry, highlighting the real-world practices and strategies used.

==> Discussion.tex <==

\section{Discussion}
\label{Discussion}

In the context of integrating HF requirements into product development, our study explores a series of propositions that evaluate the essence of effective HF management strategies through the lense of Requirements Strategy. The results provides a schematic representation of the relationships and implications of these propositions.


 \paragraph{Impact of Ownership and Responsibility on HF Integration}

The results indicate general support confirming that
clear ownership and responsibility (Proposition 1) benefit HF
integration in product development, resonating with Smith and
Reinertsen’s \cite{smith1997developing} observations on role clarity. It was discussed by interviewees that organizations may adopt a generic responsibility framework or tailor their approach to specific projects. This aligns with the findings of Cockburn \cite{cockburn2006agile}, who highlight the impact of organizational culture on the adoption of agile practices. Another critical insight emerged from the data suggesting that the responsibility often defaults to the developers.
%
For Proposition 2, the opinions on assigning HF expertise to critical roles were divergent. Some evidence favored allocating HF responsibilities to critical roles, while others advocated for the distribution of HF expertise across various supporting roles, such as to external HF teams. Interviews also highlighted a trend towards democratizing HF responsibility, suggesting that involving the entire product team in HF could improve integration and product cohesion.



\paragraph{Impact of Requirement Structuring and Information Models on HF Integration in AV Development}

The mixed perspectives on the impact of clear requirements structure on HF integration (Proposition 3) echo challenges in software requirement engineering \cite{sommerville2011software}. 
This complexity echoes the broader discourse in software engineering, where structured approaches, while valuable, must be flexible enough to accommodate the dynamic nature of product development, as noted by Cooper et al. \cite{cooper2014face}.
We identify three strategies for adoption: specialized HF structures, reliance on current robust structures, and the enhancement of existing structures with HF labels. This variety highlights organizational adaptability in integrating HF considerations into their workflows
%
For Proposition 4, concerning the traceability of HF requirements, the findings reveal varying practices: some organizations opt for specific traceability models dedicated to HF, while others integrate these requirements into a general model, and yet others do not use traceability at all. The diversity of these approaches underscores the practical challenges of maintaining traceability in various organizational contexts. This reveals that the effectiveness of traceability in HF integration may not be universally recognized, suggesting a gap between theoretical expectations \cite{rupp2009requirements, gotel1994analysis}and practical realizations.
%
The findings on the decomposition of HF requirements in Proposition 5 show varied support. The data presents a continuum of practices, ranging from rigorous top-down decomposition to treating requirements as an emergent property in innovative domains, lacking predefined requirements \cite{hoda2018rise}. This indicates that decomposition is not a static process but one that evolves with the technological landscape and organizational strategy.




\paragraph{Impact of Work and Feature Flow on HF Integration in AV Development}

Proposition 6 explores the influence of a strong lifecycle model for HF requirements. Our study provides evidence that robust lifecycle models, including agile methodologies, significantly benefit the integration of HF. This aligns with agile methodologies which emphasize adaptability and iterative development for complex requirements, as discussed in Van Der Vyver's et al. \cite{van2003agile} and Schwaber and Beedle's \cite{schwaber2001agile} work. However, there is recognition of the need to support multiple lifecycle models to cater to the varied nature of projects, highlighting the importance of considering both short-term and long-term project scopes, influenced by factors like project size, nature, organizational culture, and scope \cite{sutherland2007scrum}.
%
Proposition 7 deliberates on the clarity of HF workstream definitions in relation to other workstreams.
The debate on integrating versus separating HF activities in agile processes, echoes Cockburn and Highsmith's view on agile methodologies' adaptability across organizational contexts \cite{cockburn2001agile}.
Integrating HF with other workstreams may improve recognition and integration, but might also limit its scope to specific areas. Conversely, external HF expertise may have broaden its reach across teams, but have less influence on decision-making. This balance between specialized knowledge and cross-functional collaboration is also discussed by Highsmith \cite{highsmith2002agile}.





==> plantuml.tex <==
@startuml

package target {

  class "HF requirements" as HFR
  class "product development" as PD

}
  HFR --> PD: integration in


class "decomposition of HF requirements" as dec

class "organizational levels" as ol

dec --> ol : corresponds with

package lifecycle {
  class "Lifecycle model for HF Req" as lcm
  class "information and knowledge flow" as flow

  lcm --> flow: affects
}

lcm -> target : (P6) strength positively impacts
note top on link #green
supported
<b>solution space:</b>
  - rely on agile methods
  - more than one lifecycle model
  - short sprints vs long iterations
end note 

package workstream {
  class "HF Workstream" as hfws

  class "Other Workstreams" as ows

  hfws --> ows: clearly defined in relation
}

workstream -> target : (P7) positively impacts
note top on link  #lightgreen
partially supported
<b>solution space:</b>
  - separated or integrated HF workstream
end note

  class "Plan for review and reflection" as RnR
  
  RnR -> target : (P8) clarity positively impacts
  note top on link #lightgreen 
  partially supported
  <b>solution space:</b>
  - explicit plan for HF or not
  end note


@enduml


## P1 and P2
@startuml

package target {

  class "HF requirements" as HFR
  class "product development" as PD

}
  HFR --> PD: integration in

class "HF ownership/responsibility" as own

own -> target : (P1) clarity positively impacts
note top on link #lightgreen
<b>support:</b> (+) 
<b>solution space:</b>
  - generic responsibilities
  - tailored to projects
  - default ownership
end note

package "Allocation of HF expertise"  as all {
class "HF expertise" as hfe

class "Critical roles" as cr

hfe --> cr : assigned to
}


(hfe, cr) ..> own : (P2) required
note top on link 
<b>support:</b> +/- 
<b>solution space:</b>
  - assign to critical roles
  - assign to supporting roles
  - everybody's responsibility
end note

@enduml

## Structure combined

@startuml

package target {

  class "HF requirements" as HFR
  class "product development" as PD

}
  HFR --> PD: integration in


class "HF req structure" as str



str -> target : (P3) clarity positively impacts
note top on link #lightgreen
<b>support:</b> (+) 
<b>solution space:</b>
  - specialized structure for HF req
  - generic req structure
  - labeling of HF req
end note

class "HF req traceability" as tr

tr -> target : (P4) clarity positively impacts
note top on link 
<b>support:</b> +/-
<b>solution space:</b>
  - provide specific traceability model for HF
  - integrated in general traceability model
  - do not use traceability for product development
end note


class "decomposition of HF requirements" as dec

class "organizational levels" as ol

dec -> ol : corresponds with


target <--- dec : (P5) positively impacts
note top on link
<b>support:</b> +/- 
<b>solution space:</b>
  - decompose top-down
  - hf requirements on highest level decomposed into system requirements (ID12)
  - treat as emergent property (ID05)
end note

@enduml

## P3
@startuml

package target {

  class "HF requirements" as HFR
  class "product development" as PD

}
  HFR --> PD: integration in

class "HF req structure" as str

str -> target : (P3) clarity positively impacts
note top on link 
<b>support:</b> (+) 
<b>solution space:</b>
  - specialized structure for HF req
  - generic req structure
  - labeling of HF req
end note

@enduml
## P4

@startuml

package target {

  class "HF requirements" as HFR
  class "product development" as PD

}
  HFR --> PD: integration in

class "HF req traceability" as tr

tr -> target : (P4) clarity positively impacts
note top on link 
<b>support:</b> +/-
<b>solution space:</b>
  - provide specific traceability model for HF
  - integrated in general traceability model
  - do not use traceability for product development
end note

@enduml

## P5

@startuml

package target {

  class "HF requirements" as HFR
  class "product development" as PD

}
  HFR --> PD: integration in


class "decomposition of HF requirements" as dec

class "organizational levels" as ol

dec --> ol : corresponds with


dec -> target : (P5) positively impacts
note top on link
<b>support:</b> +/- 
<b>solution space:</b>
  - decompose top-down
  - hf requirements on highest level decomposed into system requirements (ID12)
  - treat as emergent property (ID05)
end note

@enduml
